Convolutional Neural Opacity Radiance Fields

Photo-realistic modeling and rendering of fuzzy objects with complex opacity are critical for numerous immersive VR/AR applications, but it suffers from strong view-dependent brightness, color. In this paper, we propose a novel scheme to generate opacity radiance fields with a convolutional neural renderer for fuzzy objects, which is the first to combine both explicit opacity supervision and convolutional mechanism into the neural radiance field framework so as to enable high-quality appearance and global consistent alpha mattes generation in arbitrary novel views. More specifically, we propose an efficient sampling strategy along with both the camera rays and image plane, which enables efficient radiance field sampling and learning in a patch-wise manner, as well as a novel volumetric feature integration scheme that generates per-patch hybrid feature embeddings to reconstruct the view-consistent fine-detailed appearance and opacity output. We further adopt a patch-wise adversarial training scheme to preserve both high-frequency appearance and opacity details in a self-supervised framework. We also introduce an effective multi-view image capture system to capture high-quality color and alpha maps for challenging fuzzy objects. Extensive experiments on existing and our new challenging fuzzy object dataset demonstrate that our method achieves photo-realistic, globally consistent, and fined detailed appearance and opacity free-viewpoint rendering for various fuzzy objects.

==> secs/experiment.tex <==


\section{Experiments}
\label{sec:experiment}
We quantitatively (Tables \ref{XXX}) and qualitatively (Figs. XX and xxx) show that our method can better preserve high fidelity surface details than prior work and provide extensive ablation studies to validate our design choices (Fig \ref{xxx}). We urge the reader to view our supplementary video to better appreciate our method’s significant improvement over baseline methods when rendering novel views.

% \subsection{Datasets}


\subsection{Results}

We evaluate our method on fuzzy objects including xxx synthesis and xxx real objects in total, part of them are selected from dataset \cite{wang2020neural} under the condition of neither fur surface nor rich texture details. We also collect and render some new challenge objects with Blender and further design a capture system to acquire RGBA  multi-view real objects (as demonstrated in XXX).  


% For the synthetic data, we render models \textit{Wolf} and \textit{Hair} by positioning virtual cameras on a sphere surrounding the object and use Blender to render 450 images totally and then randomly select 300 images for training and the rest for testing. For the models \textit{Girl} and \textit{Dog}, we render 340 and 224 images with virtual cameras on a semi-sphere, and use 300 and 200 images for training. For real data, we capture two fuzzy toys: \textit{Cat} and \textit{Koala}, two real hairstyle objects: \textit{Hairstyle 1} and \textit{Hairstyle 2}. We use our capture system to acquire 420, 475, 315 and 400 images respectively. For \textit{Cat}, \textit{Koala} and \textit{Hairstyle 2}, we use 300 images for training and for \textit{Hairstyle 1} we use 250 images for training. The rest of the captured images are used for both qualitative and quantitative evaluation of novel view synthesis. The corresponding ground truth alpha mattes for synthetic data are rendered with color images while for real data they are generated by our automatic matting pipeline described in Sec.XXX. We construct the coarse 3D proxy meshes for guiding bidirectional important sampling by shape from silhouette [xxx], we generate the input foreground masks by dilating the masks obtained by setting the non-zero pixels of alpha mattes to 1 to make sure that the entire object is inside the proxy. 

% We set the image resolution as $800 \times 600$ for \textit{Girl} and \textit{Dog}, $512 \times 512 $ for \textit{Hair} and $800 \times 500$ for the rest datasets. We sample 64 points per ray, the corresponding radiance feature dimension for each ray is 256 while the density feature dimension is 64. Our CRF is implemented on a single NVIDIA TITAN RTX GPU and a 2.2GHz Intel Xeon Silver 4210 CPU. We train a CRF following our patch based regression scheme described in Sec.xxx while in inference period, we render the entire image at once given specific camera pose and intrinsic.

% It is worth to mansion that our CRF can render not only test-viewpoints but arbitrary novel views with strong view-consistency in both RGB images and alpha mattes. The view synthesis results with fine details are best viewed as videos so it is necessary to view our supplementary video. 

\begin{figure*}[!t]
\centering
  \includegraphics[width=1.0\linewidth]{pic/comparison/rgb.png}
  \caption{Free Viewpoint RGB results comparison with IBOH ~\cite{matusik2002image}, NOPC~\cite{wang2020neural} and NERF ~\cite{mildenhall2020nerf} on \textit{Cat}, \textit{Girl}, \textit{Wolf} datasets. Our method is able to reconstruct fine details on both geometry and appearance, such as \textit{Cat}'s fur texture, the pattern on \textit{Girl}'s boots and the geometric details of wolf's hair. IBOH exhibits ghosting and aliasing, NOPC exhibits excessive blurs and loss geometric details and NERF exhibits excessive noise as well as blurs.}
  \label{fig:rgb_real_comparison}
\end{figure*}

% \begin{figure*}[!t]
% \centering
%   \includegraphics[width=1.0\linewidth]{pic/rgb_syn.png}
%   \caption{RGB results comparison on synthetic dataset. }
%   \label{fig:rgb_syn_comparison}
% \end{figure*}

% 主要对比 nenrf, NOPC, 
% case: 
% synthesis: hair, wolf, girl, dog, nerf cases (*8)
% real: hair(x4), cat, koala 

\begin{figure*}[!t]
\centering
  \includegraphics[width=1.0\linewidth]{pic/comparison/real_alpha.png}
  \caption{Free Viewpoint Alpha results comparison with IBOH ~\cite{matusik2002image}, NOPC~\cite{wang2020neural} and NERF ~\cite{mildenhall2020nerf} on \textit{Cat}, \textit{Hairstyle 2} datasets. Our method can recover missing part opacity such \textit{Cat}'s beard from view-inconsistent alpha mattes as shown in first row, While IBOH fails and exhibits strong polygonal artifacts. Our method can produce sharper alpha mattes than NOPC which suffers from strong artifacts around the hair. NERF fails on our challenge \textit{Hairstyle 2} dataset.}
  \label{fig:alpha_real_comparison}
\end{figure*}

\begin{figure*}[!t]
\centering
  \includegraphics[width=1.0\linewidth]{pic/syn_alpha.png}
  \caption{Alpha results comparison on synthetic datasets. }
  \label{fig:alpha_syn_comparison}
\end{figure*}

To evaluate the above methods under the same settings of dataset, iterations, and image resolution, we retrain their models for compassion. Specifically, we use XXX and XXX image resolution for synthesis and real object respectively,  XXX and XXX images for training/test. Also, as the \textit{Neural Opacity Point Cloud (NOPC)~\cite{wang2020neural}} is taking dense point cloud as input, we sample 300,000 points for each object from the same proxy mesh with us. We use $64$ samples per ray in our model, and $128$ samples (64 in coarse and fine modules) for Nerf ~\cite{mildenhall2020nerf} training.

Fig.~\ref{fig:rgb_syn_comparison} and Fig.~\ref{fig:rgb_real_comparison} show several free-viewpoint RGB and alpha rendering results together with visual compassion v.s. most recent neural scene representation methods. We can see that the \textit{IBOH} suffers from ghosting and aliasing due to the input views are in-uniform. The \textit{NOPC} can partially generate smooth texture details with sufficient training images but still suffers from color shifting, XXX why?, their result are related blurry on the \textit{Girl} object due to sparse feature extracted from low density point cloud (???). The NERF is able to preserve low-frequency components but fails to recover high-frequency details due to the limited representation ability of the MLP network. And it is also really noisy in the fur region. This phenomenon is caused by insufficient samples on both ray direction and the ray resolutions. In contrast, our CRF is able to reconstruct fine texture and geometry details and present sharply visual results.  
 
Fig.~\ref{XXX} shows the visual discrepancies of free-viewpoint alpha maps from given discrete view samples. Compared to other methods, our CRF is able to render sharper hair on the object boundary. Note that we can easily obtain a perfect alpha map in synthesis dataset while not easy for real data, our method is not sensitive to the quality of input alpha map and is able to recover missing part from nearby view samples (as shown in xxx row of Fig. ~\ref{xxx}).
 

 
 
% We compare our CRF with IBOH~\cite{matusik2002image} and other two recently free viewpoint neural renderers (NOPC\cite{XXX} Nerf\cite{martin2020nerf})s.  

% \textit{Image-Based Opacity Hull (IBOH)~\cite{matusik2002image}} We implement our own version of the IBOH[xxx] using training images as inputs which is the same to our CRF. For fair comparison, we use our coarse mesh generated by shape from silhouette algorithm as  
% proxy for the IBOH.

% \textit{Neural Opacity Point Cloud (NOPC)~\cite{wang2020neural}} We directly use the open source official implementation to conduct our experiments. We retrain the NOPC models of the same objects \textit{Hair, Wolf, Cat} rather than use the pretrained models for fairness considering the impact of different resolutions and dataset divisions. We sample 300,000 points from the coarse proxy mesh of each object for training and set the point feature dimension to 32 as the same to the original implementation. 

% \textit{Neural Radiance Fields (NERF)~\cite{martin2020nerf}} We implement the NERF[xxx] with our own fuzzy object datasets according to the
%  description in the paper. We set near and far bounds by computing the nearest and farthest distance from the coarse mesh to each camera imaging plane. We sample 64 points per ray to train the coarse network and with 64 additional importance samples through the fine network, thus the samples number is actually twice of CRF in total. 
 
 %  Fig.~\ref{fig:alpha_real_comparison} and Fig.~\ref{fig:alpha_syn_comparison} illustrates the visual discrepancies of alpha results . It should be noticed that the ground truth alpha mattes are not coherent since they are individually generated by matting algorithm: the cat's whiskers under the sample view are classified as background. However, CRF can reconstruct the objects from the multi-view images and extract 3D aware features for rendering, which enforce the coherence across all views. 
 
\subsection{Qualitative Evaluation}

We quantitatively evaluate our method on the above dataset with PSNR, LPIPS~\cite{zhang2018perceptual} with value with VGG backbone and SSIM metric. \footnote{We computer quantity value only on foreground region (i.e., the object itself) by considering the background is not included in the final render.} As shown in Tab.~\ref{table:rgb_comparison}, we see that our CRF achieves better performance on both RGB and alpha result. Note that, we replace the LPIPS metric with \textit{Sum of Absolute Distance} (SAD) due to the alpha-like image is away from the distribution of the training set in the network based distance metric.


% We conduct quantitative comparisons on CRF versus IBOH, NOPC and NERF. Firstly we evaluate our CRF on RGB rendering foreground images in Tab.~\ref{table:rgb_comparison}. We compute PSNR, SSIM and LPIPS of $\mathbf{\alpha} * \mathbf{F}$ in the non-zero region of the ground truth alpha matte because we only consider the representation of the objects rather than the whole scenes which contain the background. As shown in Tab.~\ref{table:rgb_comparison}, our CRF achieve higher performance on every dataset than previous work. We argue that for fuzzy objects which contains rich high frequency component, LPIPS is a better metric and our method reduces the LPIPS by a large margin. For alpha mattes, Tab.~\ref{table:alpha_comparison} show comparisons using PSNR, SSIM and SAD following previous matting work[xxx]. Our CRF generates alpha mattes with significantly smaller errors than the state of the art methods.   

% NERF只能大致保留低频信息，使得图像呈现出细节模糊不清的现象，并且具有噪声。而在学习低频的同时，CRF可以很好地保留几何、纹理上的高频细节，从而渲染出与GT几乎一致的令人愉悦的细节。这是因为NERF仅仅使用一个简单的MLP网络以及有限的网络参数无法表达出高频的信息，而CRF提出的Convolutional Volume Renderer则可以通过更好的利用implicit feature 表达的信息。而同样使用CNN 渲染器的NOPC可以在去除噪声的同时部分的渲染出部分顺滑的纹理信息，但是这种生成的纹理与GT并不一致，并且图像整体发生一定程度的颜色偏移。这是由于显式地点云表达无法提供出compact,有效表达3d信息的feature, 而且有限的点数量导致了投影得到的二维feature map通常具有孔洞, 通过NR的修复导致了不真实。IBOH 尽管在物体内部能够通过邻近视角的插值保持一定程度的高频纹理细节，但是在物体边缘处有巨大的artifacts。而我们的CRF则无论是在内部还是在边缘都能够渲染出以假乱真的效果。 

% \begin{table*}[!t]
% \centering
% % \caption{alpha results comparison.}
% \begin{tabular}{ ccc ccc c ccc c cc c cc} 
% \toprule
%       &&& \multicolumn{3}{c}{\textbf{Synthesis}(RGB)} & &\multicolumn{3}{c}{\textbf{Real}(RGB)} &&  \multicolumn{2}{c}{\textbf{Synthesis}(Alpha)} & &\multicolumn{2}{c}{\textbf{Real}(Alpha)}\\[2pt] \cline{4-6}\cline{8-10}\cline{12-13}\cline{15-16}
% \specialrule{0em}{1pt}{1pt}
%       &&& $\uparrow$ PSNR& $\uparrow$ SSIM& $\downarrow$ LPIPS&& $\uparrow$ PSNR& $\uparrow$ SSIM & $\downarrow$ LPIPS && $\downarrow$SAD & $\uparrow$PSNR && $\downarrow$SAD & $\uparrow$PSNR\\
% \toprule
% \multicolumn{3}{c}{\textbf{IBOH}\cite{}}& \\
% \multicolumn{3}{c}{\textbf{NOPC}\cite{martin2020nerf}}&\\
% \multicolumn{3}{c}{\textbf{NERF}\cite{}}&\\
% \multicolumn{3}{c}{\textbf{Ours}}&\\

% \toprule
% \end{tabular}
% \end{table*}

\begin{table}[!t]
\centering
\caption{Quantitative comparisons of foreground images on different datasets.}
\resizebox{1\linewidth}{!}{
\begin{tabular}{m{6em}<{\centering} m{4em}<{\centering} c c c c} 
\toprule
Method & & IBOH & NOPC & NERF & Ours \\ [0.5ex] 
\midrule
\multirow{3}{*}{\bf Wolf}           & PSNR  & 28.25 & 29.95 & 32.56 & \textbf{37.23} \\ 
                                    & SSIM  & 0.932 & 0.945 & 0.965 & \textbf{0.975} \\
                                    & LPIPS & 0.073 & 0.058 & 0.061 & \textbf{0.022} \\
\midrule
\multirow{3}{*}{\bf Hair}           & PSNR  & 23.22 & 28.31 & 28.29 & \textbf{33.56} \\ 
                                    & SSIM  & 0.872 & 0.912 & 0.932 & \textbf{0.952} \\
                                    & LPIPS & 0.104 & 0.058 & 0.070 & \textbf{0.021} \\
\midrule
\multirow{3}{*}{\bf Girl}           & PSNR  & 18.32 & 26.97 & 29.77 & \textbf{32.17} \\ 
                                    & SSIM  & 0.863 & 0.922 & 0.951 & \textbf{0.958} \\
                                    & LPIPS & 0.150 & 0.099 & 0.052 & \textbf{0.035} \\
\midrule
\multirow{3}{*}{\bf Dog}            & PSNR  & 22.53 & 27.88 & 29.59 & \textbf{31.87} \\ 
                                    & SSIM  & 0.866 & 0.902 & 0.937 & \textbf{0.950} \\
                                    & LPIPS & 0.127 & 0.098 & 0.053 & \textbf{0.030} \\
\midrule
\multirow{3}{*}{\bf Koala}          & PSNR  & 24.41 & 25.45 & 32.90 & \textbf{33.48} \\ 
                                    & SSIM  & 0.871 & 0.890 & 0.960 & \textbf{0.965} \\
                                    & LPIPS & 0.103 & 0.117 & 0.053 & \textbf{0.023} \\
\midrule
\multirow{3}{*}{\bf Cat}            & PSNR  & 20.40 & 26.72 & 24.80 & \textbf{28.95} \\ 
                                    & SSIM  & 0.810 & 0.888 & \textbf{0.896} & \textbf{0.894} \\
                                    & LPIPS & 0.198 & 0.101 & 0.187 & \textbf{0.090} \\
\midrule
\multirow{3}{*}{\bf Hairstyle 1}    & PSNR  & 25.32 & 27.34 & 17.84 & \textbf{30.51} \\ 
                                    & SSIM  & 0.905 & 0.921 & 0.904 & \textbf{0.949} \\
                                    & LPIPS & 0.067 & 0.058 & 0.135 & \textbf{0.037} \\
\midrule
\multirow{3}{*}{\bf Hairstyle 2}    & PSNR  & 25.86 & 31.14 & 19.38 & \textbf{37.21} \\ 
                                    & SSIM  & 0.951 & 0.962 & 0.931 & \textbf{0.983} \\
                                    & LPIPS & 0.104 & 0.033 & 0.131 & \textbf{0.014} \\
\bottomrule
\end{tabular}
}
\label{table:rgb_comparison}
\end{table}

\begin{table}[!t]
\centering
\caption{Quantitative comparisons of alpha mattes on different datasets}
\resizebox{1\linewidth}{!}{
\begin{tabular}{m{6em}<{\centering} m{4em}<{\centering} c c c c} 
\toprule
Method & & IBOH & NOPC & NERF & Ours \\ [0.5ex] 
\midrule
\multirow{3}{*}{\bf Wolf}           & SAD  & 18.46 & 7.977 & 4.777 & \textbf{2.564} \\ 
                                    & PSNR & 25.10 & 29.03 & 32.14 & \textbf{38.63} \\
                                    & SSIM & 0.956 & 0.983 & 0.990 & \textbf{0.996} \\
\midrule
\multirow{3}{*}{\bf Hair}           & SAD  & 18.93 & 6.117 & 5.078 & \textbf{2.077} \\ 
                                    & PSNR & 21.87 & 29.54 & 28.25 & \textbf{36.35} \\
                                    & SSIM & 0.930 & 0.981 & 0.981 & \textbf{0.994} \\
\midrule
\multirow{3}{*}{\bf Girl}           & SAD  & 48.61 & 12.66 & 5.290 & \textbf{2.877} \\ 
                                    & PSNR & 19.59 & 27.83 & 30.58 & \textbf{36.39} \\
                                    & SSIM & 0.937 & 0.986 & 0.991 & \textbf{0.996} \\
\midrule
\multirow{3}{*}{\bf Dog}            & SAD  & 30.77 & 11.32 & 6.828 & \textbf{3.661} \\ 
                                    & PSNR & 22.77 & 27.78 & 30.41 & \textbf{36.52} \\
                                    & SSIM & 0.945 & 0.983 & 0.988 & \textbf{0.995} \\
\midrule
\multirow{3}{*}{\bf Koala}          & SAD  & 26.04 & 71.32 & 190.15 & \textbf{18.94} \\ 
                                    & PSNR & 22.04 & 21.76 & 14.56 & \textbf{30.26} \\
                                    & SSIM & 0.939 & 0.962 & 0.904 & \textbf{0.983} \\
\midrule
\multirow{3}{*}{\bf Cat}            & SAD  & 50.85 & 21.46 & \textbf{20.81} & 23.79 \\ 
                                    & PSNR & 19.17 & \textbf{25.67} & 24.25 & \textbf{25.52} \\
                                    & SSIM & 0.913 & 0.958 & \textbf{0.960} & 0.944 \\
\midrule
\multirow{3}{*}{\bf Hairstyle 1}    & SAD  & 15.51 & 9.761 & 30.66 & \textbf{5.445} \\ 
                                    & PSNR & 25.06 & 28.96 & 18.16 & \textbf{32.48} \\
                                    & SSIM & 0.961 & 0.977 & 0.947 & \textbf{0.987} \\
\midrule
\multirow{3}{*}{\bf Hairstyle 2}    & SAD  & 7.677 & 5.948 & 22.69 & \textbf{2.612} \\ 
                                    & PSNR & 28.80 & 32.01 & 19.46 & \textbf{37.54} \\
                                    & SSIM & 0.980 & 0.988 & 0.957 & \textbf{0.994} \\
\bottomrule
\end{tabular}
}
\label{table:alpha_comparison}
\end{table}

\begin{table}[!t]
\centering
\caption{Ablation studies. }
\begin{tabular}{cccccccccc}
\toprule
\multicolumn{4}{c}{\multirow{2}{*}{Models}} & \multicolumn{2}{c}{$\alpha \mathbf{F}$} & \multicolumn{2}{c}{Alpha} \\\cline{5-8}
\specialrule{0em}{1pt}{1pt}
\multicolumn{4}{c}{}                        & PSNR $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SAD $\downarrow$ \\
\midrule
\multicolumn{4}{l}{(1) CRF}                     & \textbf{37.23} & \textbf{0.022} & \textbf{38.63} & \textbf{2.564} \\
\multicolumn{4}{l}{(2) w/o GAN}                 & \textbf{37.55} & 0.026& 37.93 & 2.642 \\
\multicolumn{4}{l}{(3) w/o GAN, CVR}            & 31.38 & 0.074 & 34.46 & 3.808 \\
\multicolumn{4}{l}{(4) w/o GAN, CVR, BIS}       & 20.27 & 0.175 & 20.18 & 23.51 \\
\bottomrule
\end{tabular}
\label{table:ablation}
\end{table}





% quality 
% 量化

% ablation study
% loss, gan

\begin{figure*}[!t]
\centering
  \includegraphics[width=1.0\linewidth]{pic/ablation/ablation_wolf.pdf}
  \caption{Ablation study. }
  \label{fig:ablation}
\end{figure*}


\subsection{Ablation Study}
% module 1) ray sampling 2) unet 3) gan
% loss 1) feature loss 2) composite loss 
To explore the contribution of each part in our pipeline, we conduct ablation studies by choosing a set of controlled experiments including random ray sampling v.s. important sampling, MLP based ray renderer v.s. convolutional renderer and with/without GAN based discriminator loss. 

% To evaluate different modules of our framework and training strategies, we also conduct ablation study on synthetic data \textit{Wolf} as shown in Fig.~\ref{fig:ablation} and show quantitative comparisons between different models in Tab.~\ref{table:ablation}. 

\textbf{Random v.s. Bidirectional Important Sampling} We firstly evaluate the proposed Bidirectional Important Sampling (BIS) scheme ~\ref{secXXX}. We first train a baseline model(i.e., \textit{NERF}) with 64 samples per ray, same as our CRF and a model \textit{CRF-D} with BIS. As the \textit{Wolf} case shown in Fig.~\ref{fig:ablation}, \textit{NERF} fails to recover surface details while BIS brings significant improvements to the visual quality and quantitative quality shown by model (3) and (4) in Tab.~\ref{table:ablation}.

\textbf{MLP v.s. Convolutional Renderer} We train our generator model \textit{CRF-R} only without discriminator to evaluate the effect of our Convolutional Volume Renderer(CVR). For visual comparison in Fig.~\ref{fig:ablation}, \textit{CRF-R} can synthesize fine texture details on the wolf's forehead while \textit{CRF-D} can only preserve low frequency information. CVR further improves the image quality as shown by model (2) and (3) in Tab.~\ref{table:ablation}.  

\textbf{W/o GAN Loss} We further evaluate the effect of the GAN framework adopted for fine details refinement. We compare our full \textit{CRF} model with \textit{CRF-R} model. The synthetic details of \textit{CRF-R} are a little over-smoothed while \textit{CRF} can synthesize fine and sharp details like fur texture and hairlines, which is almost the same as the ground truth. As for quantitative metrics, \textit{CRF} keep high performance on foreground image and further improve alpha quality, as shown by model (1) and (2) in Tab.~\ref{table:ablation}.

% NERF-32 represents the original NERF model trained with 32 samples per ray through coarse network and 32 importance samples through fine network, which is the same samples number with our CRF in total. CRF-D denotes the NERF model trained using our proposed Bidirectional Important Sampling scheme. CRF-R represents our generator model that adopts our convolutional volume renderer to render the implicit features to rgb images and alpha mattes. CRF-W is our entire CRF model. As shown in Fig.~\ref{fig:ablation}, NERF-32 fails to render satisfactory
% image without any details on \textit{Wolf} data, and exhibits a lot of noise and blur on \textit{Hairstyle 1}. CRF-D can effectively reduces noise and preserve the low frequency component information correctly. CRF-R can synthesize fine texture details on the wolf's forehead, but compare to the ground truth, the synthetic details are a litte over-smoothed and exhibits color bleeding phenomenon on the hair boundary. Our full model CRF-W can preserve high frequency information and as a result can synthesize fine and sharp details like fur texture and hairlines, which is almost the same to the ground truth.  
\begin{figure}[!t]
\centering
    \includegraphics[width=1.0\linewidth]{pic/cure.pdf}
\caption{First row: synthesis quality vs. sample numbers, second row: synthesis quality vs. training image number}
\label{fig:sample_numbers_curve}
\end{figure}

\begin{figure}[!t]
\centering
    \includegraphics[width=1.0\linewidth]{pic/blank.png}
\caption{synthetic quality v.s. training patch size. }
\label{fig:sample_numbers_curve}
\end{figure}

\textbf{Sampling Number.} We further demonstrate the effect of sampling different number points per ray. We sample $N \in \{16, 32, 48, 64\}$ per ray in total to train 4 different CRF models on \textit{Hairstyle 1}, and conduct quantitative evaluation as shown in Fig.~\ref{fig:sample_numbers_curve}. It is not strange that more sample points lead to higher synthesis image quality and higher alpha prediction accuracy since it helps reconstruct fine geometry details such as hairlines. However, notice that our method can still produce satisfactory results even with a few samples per ray, which can reduce the rendering time. 

\textbf{Training Size.} We randomly sample subsets of the training data \textit{Hairstyle 1} of different size $S \in \{50, 100, 150, 200, 250\}$ to train our model. Fig.~\ref{fig:image_number_curve} shows the quantitative comparison. Our model can produce relatively high quality synthesis foreground images with sparse training data, while the alpha quality increases as the number of training images increases.


\subsection{Limitation}
Unlike other objects, accurate reconstruction and rendering of furry objects requires high quality camera calibration. As our method relies on 3D implicit volumetric geometry reconstructed from 2D images, inaccurate camera poses will lead to loss of geometric details and reduce the quality of synthesis images. Thus it may fail on data captured by hand-held devices. On the other hand, since our method requires background image captured or separated by matting algorithms, it is almost impossible to manually capture the aligned background or obtain accurate alpha matte of images with complex background. So one limitation of our approach is that it is hard to applied to in the wild data.

Another limitation is that our method struggles with modeling specular objects though it can preserve view-dependent effect. This is due to that convolutional neural network fuses the features of a local patch and prediction the entire image in the same time rather than per ray prediction. In addition, the use of GAN framework enables our model to preserve high frequency image details, however, it also introduces a slight view inconsistency such as color flashes slightly between smoothly moved viewpoints. 


